The effect of weak magnetic photon emission from quark-gluon plasma

We propose a novel effect that accounts for the photon emission from a quark-gluon plasma in the presence of a weak external magnetic field. Although the weak magnetic photon emission from quark-gluon plasma only leads to a small correction to the photon production rate, the induced photon spectrum can be highly azimuthally anisotropic, as a consequence of the coupled effect of the magnetic field and the longitudinal dynamics in the background medium. With respect to a realistic medium evolution containing a tilted fireball configuration, the direct photon elliptic flow from experiments is reproduced. In comparison to the experimental data of direct photon elliptic flow, in heavy-ion collisions the magnitude of the magnetic field before 1 fm/c can be extracted. For the top energy of RHIC collisions, right after the pre-equilibrium evolution, $|eB|$ is found no larger than a few percent of the pion mass square.

==> code/source/music_input <==
###################################
# parameters list
###################################
#
echo_level  1   # control the mount of message output to screen
mode 2   # MUSIC running mode
         # 1: Does everything. Evolution. Computation of thermal spectra. 
         #    Resonance decays. Observables.  
         #    Only compatible with freeze_out_method=3 and pseudofreeze=1
         # 2: Evolution only.
         # 3: Compute all thermal spectra only.
         # 4: Resonance decays only.
         # 13: Compute observables from previously-computed thermal spectra
         # 14: Compute observables from post-decay spectra
#
#
###################################
# parameters for initial conditions
###################################
Initial_profile 1               # type of initial condition 
                                # 0: for Gubser flow test (future)
                                # 1: Optical Glauber model
                                # 3: MC-Glauber model
                                # 8: Read in initial profile from a file 
                                #    (e.g., IP-Glasma)
initialize_with_entropy 1       # 0: with energy density 
                                # 1: with entropy density

# read in initial conditions from external file
Initial_Distribution_input_filename example_inputs/filename    
                               # the filename of initial profile 
                               # (for Initial_profile == 8)
s_factor 28.66                   # normalization factor read in 
                               # initial data file
Eta_plateau_size 20.           # size of the plateau in eta_s
Eta_fall_off 0.7               # the scale of the fall off of the 
                               # plateau in eta_s direction
#
# parameters for Glauber model (effective only when Initial_profile == 1)
binary_collision_scaling_fraction 0.15    # for wounded nucleon/binary 
                                          # collision mixing ratio in the 
                                          # Glauber model
Maximum_energy_density 54.                # maximum energy density for Glauber 
                                          # initial condition
SigmaNN 42.1                              # NN inelastic cross section for 
                                          # Glauber model
Impact_parameter 10.5                       # impact parameter (fm)
Target Au                                 # type of target nucleus
Projectile Au                             # type of projectile nucleus
# parameters for Glauber model (effective only when Initial_profile == 1)
sigma_0 0.4                               # the width of the gaussian
                                          # for entropy density profile
bmin 0.0                                  # minimum value of impact parameter
bmax 2.0                                  # maximum value of impact parameter
#
#
#######################################
# parameters for hydrodynamic evolution
#######################################
boost_invariant  0            # whether the simulation is boost-invariant 
# grid information
Initial_time_tau_0 0.4        # starting time of the hydrodynamic 
                              # evolution (fm/c)
Total_evolution_time_tau 10.  # the maximum allowed running 
                              # evolution time (fm/c)
                              # need to be set to some large number
Delta_Tau 0.1                # time step to use in the evolution [fm/c]
Eta_grid_size 20.0            # spatial rapidity range 
                              # [-Eta_grid_size/2, Eta_grid_size/2 - delta_eta]
Grid_size_in_eta 64            # number of the grid points in spatial 
                              # rapidity direction
                              # Must have at least 4 cells per processor.
                              # Must be an even number.
                              # One cell is positioned at eta=0, 
                              # half the cells are at negative eta,
                              # the rest (one fewer) are at positive eta
X_grid_size_in_fm 20.0        # spatial range along x direction in the 
                              # transverse plane 
                              # [-X_grid_size_in_fm/2, X_grid_size_in_fm/2]
Y_grid_size_in_fm 20.0        # spatial range along y direction in the 
                              # transverse plane 
                              # [-Y_grid_size_in_fm/2, Y_grid_size_in_fm/2]
Grid_size_in_y 64            # number of the grid points in y direction
Grid_size_in_x 64            # number of the grid points in x direction
#
#
EOS_to_use 7                  # type of the equation of state
                              # 0: ideal gas
                              # 1: EOS-Q from azhydro
                              # 2: lattice EOS s95p-v1 
                              #    (from Huovinen and Petreczky)
                              # 3: lattice EOS s95p with partial 
                              #    chemical equilibrium (PCE) at 150 MeV 
                              #    (see https://wiki.bnl.gov/TECHQM
                              #         /index.php/QCD_Equation_of_State)
                              # 4: lattice EOS s95p with chemical freeze 
                              #    out at 155 MeV
                              # 5: lattice EOS s95p at 160 MeV
                              # 6: lattice EOS s95p at 165 MeV
                              # 7: lattice EOS s95p-v1.2 for UrQMD
reconst_type  1               # 0: solve energy density for hydro eqns.
                              # 1: solve flow velocity for hydro eqns.
Minmod_Theta 1.8              # theta parameter in the min-mod like limiter
Runge_Kutta_order 2           # order of Runge_Kutta for temporal evolution 
                              # (must be 1 or 2)
# transport coefficients
Viscosity_Flag_Yes_1_No_0 1        # turn on viscosity in the evolution
Include_Shear_Visc_Yes_1_No_0 1    # include shear viscous effect
Shear_to_S_ratio 0.095              # value of \eta/s
T_dependent_Shear_to_S_ratio  0    # flag to use temperature dep. \eta/s(T)
Include_Bulk_Visc_Yes_1_No_0 0     # include bulk viscous effect
Include_second_order_terms 0       # include second order non-linear coupling terms
#
#
# switches to output evolution information
output_evolution_data 1            # flag to output evolution history to file
outputBinaryEvolution  0           # output evolution file in binary format
output_evolution_every_N_eta  1    # output evolution file every Neta steps
output_evolution_every_N_y  1      # output evolution file every Ny steps
output_evolution_every_N_x  1      # output evolution file every Nx steps
output_evolution_every_N_timesteps  1  # output evolution every Ntime steps
#
#
###########################################
# parameters for freeze out and Cooper-Frye 
###########################################
Do_FreezeOut_Yes_1_No_0 0       # flag to find freeze-out surface
freeze_out_method 2             # method for hyper-surface finder
                                # 2: Schenke's more complex method
average_surface_over_this_many_time_steps 5   # the step skipped in the tau
epsilon_freeze 0.18             # the freeze out energy density (GeV/fm^3)
use_eps_for_freeze_out 1        # flag to use energy density as criteria to 
                                # find freeze-out surface 
                                # 0: use temperature, 1: use energy density
T_freeze 0.135                  # freeze-out temperature (GeV)
#
#
EndOfData

